Analyzing COVID-19 Tweets with Transformer-based Language Models

This paper describes a method for using Transformer-based Language Models (TLMs) to understand public opinion from social media posts. In this approach, we train a set of GPT models on several COVID-19 tweet corpora that reflect populations of users with distinctive views. We then use prompt-based queries to probe these models to reveal insights into the biases and opinions of the users. We demonstrate how this approach can be used to produce results which resemble polling the public on diverse social, political and public health issues. The results on the COVID-19 tweet data show that transformer language models are promising tools that can help us understand public opinions on social media at scale.

==> text/how_we_feel.tex <==
\subsubsection{PROBES: How we feel}
We created explicitly subjective probes to see if there would be any difference between the results of probes that use the subjective \enquote{I} and \enquote{we} when compared to the specific groups of the previous section. The two probes were \enquote{During the pandemic, I've/we've been feeling}. For the \enquote{we've been feeling} probe, the results are substantially similar to the \enquote{Americans} probe in Figure~\ref{fig:asian_black_americans_feeling}. The main difference between the results of these two probes was the granularity of the response. To get to the same percentage of responses (approximately 500 out of 1,000), 17 terms rather than 6 had to be summed (Figure~\ref{fig:ive_been_feeling_top_50_perc}). 

\begin{figure}[h]
	\centering
	\fbox{\includegraphics[width=22em]{figures/Ive_been_feeling_top_50_perc}}
	\caption{\label{fig:ive_been_feeling_top_50_perc} I've been feeling, top terms}
\end{figure}
\shimei{In the above figure, it contains only the I've been feeling results (as suggested by the caption) or a combined I/we have been feeling results? Why not include the results in this figure to Figure 1 to directly compare Americans versus we versus I?}

Self-referential responses are more varied than group-referential regardless of whether the writer perceives themselves as part of the group or not. This diversity in the generated responses include negative examples such as \enquote{During the pandemic, I’ve been feeling \textit{more depressed, confused, and scared.}}, and positive, such as \enquote{During the pandemic, I’ve been feeling \textit{more grateful and hopeful than ever.}} 
\shimei{The above paragraph is to compare "I" versus "We" or "We" versus "Americans"? In your example, you only have "I". It is unclear the exact point you want to make in the above paragraph}
\phil{Let's discuss in today's meeting. Individual responses are more granular, but maybe this is a good part to delete}

==> text/man_woman.tex <==
We can illustrate how GPT generates texts that are sensitive to and consistent with given prompts with the following two examples. In each case the model\footnote{Text generated using the OpenAI beta GPT-3 playground} generates 100 tokens of text based on the prompt  \enquote{the wo/man walked into the room}.

\begin{displayquote}
	\textbf{GPT-3 text sample 1:}The woman walked into the room \textit{and sat down on the bed. She was a little older than me, maybe in her late twenties. She had long, dark hair and a pretty face. She was wearing a white blouse and a black skirt. She looked like a secretary.}
\end{displayquote}

\begin{displayquote}
	\textbf{GPT-3 text sample 2:}The man walked into the room \textit{and sat down in the chair across from her. He was a big man, with a thick neck and a bald head. He wore a black suit and a white shirt.}
\end{displayquote}

Even though the starting prompts differ only by one word, and the generated text starts with the same words, the trajectories are quite different. Because of this ability to synthesize responses that are consistent with prompts, GPTs could provide capabilities for capturing the human opinions and beliefs encoded in the training text that more resemble the traditional polling model. Rather than performing traditional text mining (e.g., supervised classification), we can \textit{poll} the model's responses to probes. But to do this effectively requires that we develop methods to systematically reveal the relevant latent information captured in these models.
%In the first sample, the text includes terms that emphasize traditional gender stereotypes, the subject is \enquote{pretty}, with \enquote{long dark hair} who looks \enquote{like a secretary}. In the second sample, the subject is described in equivalent male stereotypes. He is a \enquote{big man} with a \enquote{thick neck} which can imply strength.\jimmy{In US English, periods and commas are supposed to be inside quotation marks.  It's illogical but it was done to increase the lifespan of typewriters.  If you need to save space, this paragraph could be removed or condensed.  The reader can draw their own conclusions and doesn't really need to see our opinion on it.} 

\begin{comment}
We can repeat these prompts and get different results by adjusting the \textit{temperature} of the model. This introduces a level of randomness in which high-ranking token is used for the next word. Using the same prompt with a temperature of 0.7, we now get a more extreme divergence in the gendered description: 

GPT-3 text sample 3:
\begin{displayquote}
\textit{\textbf{The woman walked into the room} and stood across from me. She had long dark hair that fell past her shoulders and matched her black dress that was covered in a sheer fabric that made the outline of her body visible. Her heels were so high, they made her legs look longer than they already were. Her eyes were dark and deep, and they matched her hair. She smiled, lips painted red to match her dress and shoes.}
\end{displayquote}

GPT-3 text sample 4:
\begin{displayquote}
\textit{\textbf{The man walked into the room} and stood in front of her. He pulled back the sheet that was covering her and grabbed her breast. Then he pulled off his pants and forced her hand down his underwear.}
\end{displayquote}
\end{comment}

%These texts imply that gender-specific spaces exist in the model, and that they can be explored  using textual prompts. %The behavior of the model can be influenced by parameters such as sampling probability, temperature, and search strategy \cite{holtzman2019curious}. The text output of the model is a novel synthesis of the information in the model in a complex interaction with these rules. 
